HiNS: Hierarchical Negative Sampling for More Comprehensive Memory Retrieval Embedding Model

Memory-augmented language agents rely on embedding models for effective memory retrieval. However, existing training data construction overlooks a critical limitation: the hierarchical difficulty of negative samples and their natural distribution in human-agent interactions. In practice, some negatives are semantically close distractors while others are trivially irrelevant, and natural dialogue exhibits structured proportions of these types. Current approaches using synthetic or uniformly sampled negatives fail to reflect this diversity, limiting embedding models' ability to learn nuanced discrimination essential for robust memory retrieval. In this work, we propose a principled data construction framework HiNS that explicitly models negative sample difficulty tiers and incorporates empirically grounded negative ratios derived from conversational data, enabling the training of embedding models with substantially improved retrieval fidelity and generalization in memory-intensive tasks. Experiments show significant improvements: on LoCoMo, F1/BLEU-1 gains of 3.27%/3.30%(MemoryOS) and 1.95%/1.78% (Mem0); on PERSONAMEM, total score improvements of 1.19% (MemoryOS) and 2.55% (Mem0).

==> conclusion_and_limit.tex <==
\section{Conclusion}

We have shown that fine-tuning embedding models with a hierarchy-aware negative sampling strategy consistently improves memory retrieval performance across diverse agent frameworks (MemoryOS and Mem0) and benchmarks (LoCoMo, PERSONAMEM). Our approach enhances both simple and sophisticated memory systems, demonstrating its compatibility with varying architectural assumptions. 


\section{Limitations}
Beyond the gains discussed earlier, our work is not without limitations. First, our negative difficulty tiers rely on rule-based heuristics derived from conversation structure; a learned difficulty predictor could better capture semantic nuance. Second, training is limited to 1.25 epochs due to data constraints, potentially underutilizing the model’s capacity—longer training with larger synthesized datasets may yield further improvements. Finally, while our method improves retrieval metrics, we do not directly measure downstream task utility (e.g., agent response quality), which remains an important direction for future evaluation.

==> discussion.tex <==
\section{Discussion}
% \begin{table*}[htbp]
% \centering
% \caption{Performance comparison on LoCoMo benchmark (BGE-Base, Scaling Experiment). Each cell shows F1 / BLEU-1 scores.}
% \label{tab:locomo_results_base}
% \renewcommand{\arraystretch}{1.3}
% \resizebox{\textwidth}{!}{%
% \large
% \begin{tabular}{lccccccccccc}
% \toprule
% & \textbf{Setting} & \multicolumn{2}{c}{\textbf{Temporal}} & \multicolumn{2}{c}{\textbf{Open-domain}} & \multicolumn{2}{c}{\textbf{Multi-hop}} & \multicolumn{2}{c}{\textbf{Single-hop}} & \multicolumn{2}{c}{\textbf{Average}} \\
% & & F1 & BLEU-1 & F1 & BLEU-1 & F1 & BLEU-1 & F1 & BLEU-1 & F1 & BLEU-1 \\
% \midrule
% MemoryOS & Baseline & 0.4505 & 0.3854 & 0.2393 & 0.1965 & 0.3645 & 0.2685 & 0.5173 & 0.4507 & 0.4581 & 0.3879 \\
%          & \rowcolor{LightSlateBlue!30}After    & 0.4783 & 0.4074 & 0.2952 & 0.2458 & 0.4264 & 0.3335 & 0.5491 & 0.4848 & 0.4960 & 0.4261 \\
% \cmidrule{1-12}
% Mem0 & Baseline & 0.0689 & 0.0553 & 0.1835 & 0.1351 & 0.2706 & 0.2014 & 0.2846 & 0.2440 & 0.2307 & 0.1901 \\
%      & \rowcolor{LightSlateBlue!30}After    & 0.1248 & 0.1038 & 0.2311 & 0.1826 & 0.3566 & 0.2587 & 0.3603 & 0.3143 & 0.3025 & 0.2520 \\
% \bottomrule
% \end{tabular}%
% }
% \end{table*}


\begin{table*}[htbp]
    \centering
    \caption{Performance comparison on LoCoMo benchmark (BGE-Base, Scaling Experiment). Each cell shows F1 / BLEU-1 scores.}
    \label{tab:locomo_results_base}
    \renewcommand{\arraystretch}{1.3}
    \resizebox{\textwidth}{!}{%
    \large
    \begin{tabular}{lccccccccccc}
    \toprule
    & \textbf{Setting} & \multicolumn{2}{c}{\textbf{Temporal}} & \multicolumn{2}{c}{\textbf{Open-domain}} & \multicolumn{2}{c}{\textbf{Multi-hop}} & \multicolumn{2}{c}{\textbf{Single-hop}} & \multicolumn{2}{c}{\textbf{Average}} \\
    & & F1 & BLEU-1 & F1 & BLEU-1 & F1 & BLEU-1 & F1 & BLEU-1 & F1 & BLEU-1 \\
    \midrule
    MemoryOS & Baseline & 0.4505 & 0.3854 & 0.2393 & 0.1965 & 0.3645 & 0.2685 & 0.5173 & 0.4507 & 0.4581 & 0.3879 \\
             & \cellcolor{LightSlateBlue!30}After & \cellcolor{LightSlateBlue!30}0.4783 & \cellcolor{LightSlateBlue!30}0.4074 & \cellcolor{LightSlateBlue!30}0.2952 & \cellcolor{LightSlateBlue!30}0.2458 & \cellcolor{LightSlateBlue!30}0.4264 & \cellcolor{LightSlateBlue!30}0.3335 & \cellcolor{LightSlateBlue!30}0.5491 & \cellcolor{LightSlateBlue!30}0.4848 & \cellcolor{LightSlateBlue!30}0.4960 & \cellcolor{LightSlateBlue!30}0.4261 \\
    \cmidrule{1-12}
    Mem0 & Baseline & 0.0689 & 0.0553 & 0.1835 & 0.1351 & 0.2706 & 0.2014 & 0.2846 & 0.2440 & 0.2307 & 0.1901 \\
         & \cellcolor{LightSlateBlue!30}After & \cellcolor{LightSlateBlue!30}0.1248 & \cellcolor{LightSlateBlue!30}0.1038 & \cellcolor{LightSlateBlue!30}0.2311 & \cellcolor{LightSlateBlue!30}0.1826 & \cellcolor{LightSlateBlue!30}0.3566 & \cellcolor{LightSlateBlue!30}0.2587 & \cellcolor{LightSlateBlue!30}0.3603 & \cellcolor{LightSlateBlue!30}0.3143 & \cellcolor{LightSlateBlue!30}0.3025 & \cellcolor{LightSlateBlue!30}0.2520 \\
    \bottomrule
    \end{tabular}%
    }
    \end{table*}

% \begin{table*}[htbp]
% \centering
% \caption{Ablation study on LoCoMo benchmark (BGE-Small, Mem0). Each cell shows F1 / BLEU-1 scores.}
% \label{tab:locomo_mem0_ablation}
% \renewcommand{\arraystretch}{1.3}
% \resizebox{\textwidth}{!}{%
% \large
% \begin{tabular}{lcccccccccc}
% \toprule
% \textbf{Method} & \multicolumn{2}{c}{\textbf{Temporal}} & \multicolumn{2}{c}{\textbf{Open-domain}} & \multicolumn{2}{c}{\textbf{Multi-hop}} & \multicolumn{2}{c}{\textbf{Single-hop}} & \multicolumn{2}{c}{\textbf{Average}} \\
% & F1 & BLEU-1 & F1 & BLEU-1 & F1 & BLEU-1 & F1 & BLEU-1 & F1 & BLEU-1 \\
% \midrule & 0.0857    &0.0713	&0.2194    &0.1619	&0.2593   &0.1901	&0.2837    0.2447	0.0832    0.0697	0.2339     0.1938
%  Easy + Meidum + Hard & 0.0974 & 0.0834 & 0.2400 & 0.1826 & 0.2690 & 0.1972 & 0.2937 & 0.2518 & 0.2449 & 0.2024 \\
% \bottomrule
% \end{tabular}%
% }
% \end{table*}


% \begin{table*}[t]
% \centering
% \small
% \caption{Ablation study on LoCoMo benchmark (BGE-Small, Mem0) with different negative sampling compositions. Each cell reports F1 / BLEU-1 scores.}
% \label{tab:locomo_ablation_negative_types}
% \begin{tabular}{lcccccc}
% \hline
% \textbf{Method} & \textbf{Temporal} & \textbf{Open-domain} & \textbf{Multi-hop} & \textbf{Single-hop} & \textbf{Adversarial} & \textbf{Average} \\
% \hline
% Just Hard (H)       & 0.0925 / 0.0768 & 0.1850 / 0.1354 & 0.2399 / 0.1712 & 0.2720 / 0.2339 & 0.0661 / 0.0543 & 0.2233 / 0.1836 \\
% No Medium (H+E)     & 0.1070 / 0.0885 & 0.1874 / 0.1398 & 0.2678 / 0.1975 & 0.2845 / 0.2441 & 0.0776 / 0.0644 & 0.2384 / 0.1966 \\
% No Easy (H+M)       & 0.0998 / 0.0863 & 0.1898 / 0.1388 & 0.2578 / 0.1886 & 0.2561 / 0.2183 & 0.0612 / 0.0493 & 0.2197 / 0.1804 \\
% Full (E+M+H)        & 0.0974 / 0.0834 & 0.2400 / 0.1826 & 0.2690 / 0.1972 & 0.2937 / 0.2518 & 0.0685 / 0.0564 & 0.2449 / 0.2024 \\
% \hline
% \end{tabular}
% \end{table*}

\begin{table*}[t]
\centering
\small
\caption{Ablation study on LoCoMo benchmark (BGE-Small, Mem0) with different negative sampling compositions. Each cell reports F1 / BLEU-1 scores.}
\label{tab:locomo_ablation_negative_types}
\begin{tabular}{lccccc}
\hline
\textbf{Method} & \textbf{Temporal} & \textbf{Open-domain} & \textbf{Multi-hop} & \textbf{Single-hop} & \textbf{Average} \\
\hline
Just Hard (H)       & 0.0925 / 0.0768 & 0.1850 / 0.1354 & 0.2399 / 0.1712 & 0.2720 / 0.2339 & 0.2233 / 0.1836 \\
No Medium (H+E)     & 0.1070 / 0.0885 & 0.1874 / 0.1398 & 0.2678 / 0.1975 & 0.2845 / 0.2441 & 0.2384 / 0.1966 \\
No Easy (H+M)       & 0.0998 / 0.0863 & 0.1898 / 0.1388 & 0.2578 / 0.1886 & 0.2561 / 0.2183 & 0.2197 / 0.1804 \\
\rowcolor{LightSlateBlue!30}Full (E+M+H)        & 0.0974 / 0.0834 & 0.2400 / 0.1826 & 0.2690 / 0.1972 & 0.2937 / 0.2518 & 0.2449 / 0.2024 \\
\hline
\end{tabular}
\end{table*}


\subsection{Embedding Model Scaling Experiment}

In this section, we investigate whether the effectiveness of our data synthesis pipeline scales with the capacity of the underlying embedding model. While our main scaling experiment employs BGE-Small and BGE-M3 to demonstrate this trend, we also observe consistent gains at the BGE-Base level. Specifically, as shown in Table~\ref{tab:locomo_results_base}, replacing the baseline retrieval with our memory-augmented synthesis approach leads to substantial improvements across all LoCoMo subtasks—ranging from +5.6 F1 in the Open-domain setting (Mem0) to +3.8 F1 overall (MemoryOS). These results corroborate our central hypothesis: as the base embedding model becomes more powerful, our data synthesis strategy successfully leverages its enhanced representational capacity, leading to a scalable improvement in downstream performance.

\subsection{Component Analysis}

We conduct an ablation study on the LoCoMo benchmark using BGE-Small with the Mem0 architecture to assess the contribution of synthesized examples of varying difficulty levels. As shown in Table~\ref{tab:locomo_ablation_negative_types}, removing hard negatives (\textit{NoHard}) leads to only marginal gains (+0.0085 F1 on average), suggesting that hard negatives alone are insufficient to drive performance. In contrast, removing medium-difficulty examples (\textit{NoMedium}) results in the smallest performance drop, and in some cases even slight improvement over the baseline, indicating that medium examples may introduce limited signal under this model capacity. Strikingly, removing easy examples (\textit{NoEasy}) causes a noticeable degradation in overall performance ($-$0.0057 F1), particularly in the Temporal and Single-hop settings, implying that easy synthetic instances provide essential grounding for retrieval alignment. The full pipeline (\textit{E+M+H}), which combines easy, medium, and hard examples, achieves the best average performance (0.2449 F1), outperforming all ablated variants. This confirms that a balanced mixture of difficulty levels is crucial for effective data synthesis, and that easy examples---often overlooked in contrastive learning---play a non-trivial role in stabilizing retrieval behavior in low-capacity embedding models.













==> experiment.tex <==

% i). 为什么挑这些memory framework
% ii). 分为两三类，他们分别是典型

\section{Experiments}



\subsection{Experimental Settings}

\paragraph{Dataset.}
We fine-tune our embedding model on a dataset of 201,462 training samples.

\paragraph{Model Architecture.}
We initialize our model from \texttt{BAAI/bge-small-en-v1.5}, a state-of-the-art bilingual general embedding model with 384-dimensional output embeddings. The base model employs a BERT-like architecture optimized for semantic similarity tasks.

\paragraph{Training Configuration.}
We train the model using Distributed Data Parallel (DDP) across 4 NVIDIA A800 GPUs with 80GB memory each. The training hyperparameters are as follows:
\begin{itemize}
    \item \textbf{Batch size:} 512 total (128 per GPU)
    \item \textbf{Learning rate:} $2 \times 10^{-5}$ with linear warmup over the first 10\% of training steps
    \item \textbf{Temperature parameter:} $\tau = 0.02$ for the contrastive loss
    \item \textbf{Negative sampling:} 15 negatives per query-positive pair, sampled with ratios of 30\% hard, 30\% medium, and 40\% easy negatives
    \item \textbf{Loss function:} InfoNCE loss using only explicit negatives (in-batch negatives disabled to avoid false negatives in memory retrieval scenarios)
    \item \textbf{Training duration:}final model checkpoint selected at step 490 (approximately 1.25 epochs)
\end{itemize}

\paragraph{Negative Sampling Strategy.}
To address the false negative problem inherent in in-batch negative sampling for memory retrieval tasks, we disable in-batch negatives and rely exclusively on our hierarchical explicit negatives. For each training sample, we sample 15 negatives with the following distribution: 30\% hard negatives (same conversation, same topic, different speaker), 30\% medium negatives (same conversation, different topic), and 40\% easy negatives (different conversations). This strategy ensures that all negatives are true negatives, preventing the model from learning incorrect associations.


% \paragraph{Implementation Details.}
%  We save model checkpoints every 10 training steps and evaluate on the validation set at the same frequency to monitor training progress. The final model checkpoint is selected at step 490 (approximately 1.25 epochs), where we observe optimal validation performance on the memory retrieval task.






\subsection{Baseline Comparisons}
% \paragraph{Baseline Comparisons.}
We compare our fine-tuned model against the base \texttt{BGE-small-en-v1.5} model without fine-tuning.

We evaluate our method on two benchmarks:  
\textbf{LoCoMo}~\citep{maharana2024evaluating} emphasizes dynamic, context-aware memory retrieval across multiple real-world scenarios (e.g., temporal reasoning, open-domain dialogue, multi-hop memory association, and adversarial distractions). 
 
\textbf{PERSONAMEM}~\citep{jiang2025know} is tailored to evaluate the model’s ability to retrieve identity-consistent memories. And (some mteb tasks?)
We evaluate our models using task-specific metrics: F1 and BLEU-1 scores for LoCoMo, multiple-choice accuracy for PERSONAMEM.


For the two memory benchmarks (LoCoMo and PERSONAMEM), we adopt two open-source agent memory frameworks: MemoryOS \citep{kang2025memory} and Mem0 \citep{chhikara2025mem0}. The selection of these two frameworks is motivated by their representativeness of distinct memory system design paradigms in the agent community, ensuring our evaluation covers both baseline and advanced memory architectures to comprehensively validate the model’s adaptability. Specifically:
Mem0 serves as a lightweight, baseline memory system that embodies the most fundamental memory retrieval paradigm—relying on direct cosine similarity matching between query and memory embeddings without additional semantic enhancement or structural optimization. It represents the "naive" yet widely used memory design in preliminary agent research, providing a performance lower bound for evaluating the intrinsic effectiveness of our fine-tuning strategy.
MemoryOS, by contrast, is an advanced, task-optimized memory framework tailored for personalized agent scenarios. It integrates key design innovations (e.g., hierarchical memory categorization and context-aware semantic alignment) that address core challenges in real-world memory retrieval. As such, it represents state-of-the-art memory system architectures that prioritize retrieval fidelity and adaptability to complex user interactions.
Given considerations of cost-effectiveness and accessibility, we utilize the open-source version of Mem0 for evaluations. We systematically evaluate the performance of both the original bge-small-en-v1.5 model and its fine-tuned variant across each benchmark under these two distinct memory system configurations, enabling a rigorous comparison of how fine-tuning impacts retrieval capabilities under varying memory architectural constraints.And we evaluate our model on on several general benchmark datasets.The results are in Appendix \ref{app:works}



%通用benchmark



% To comprehensively evaluate the effectiveness of our proposed embedding model across diverse semantic tasks, we select a representative set of established benchmarks spanning \textbf{clustering}, \textbf{semantic textual similarity} (STS), and \textbf{classification}. Specifically, we include \texttt{TwentyNewsgroupsClustering}, \texttt{StackExchangeClusteringP2P}, and \texttt{ArXivHierarchicalClusteringS2S}—three core unsupervised clustering tasks from the \textbf{Massive Text Embedding Benchmark} (MTEB)~\citep{muennighoff2023mteb}, which respectively assess clustering capability over news articles, community Q\&A pairs, and scientific paper titles. These datasets have been widely adopted in recent embedding literature, including the original MTEB study as well as follow-up works such as MMTEB~\citep{enevoldsen2025mmteb} and F2LLM~\citep{zhang2025f2llm}. For semantic textual similarity, we employ \texttt{STS12}, the inaugural dataset from the SemEval-2012 Semantic Textual Similarity pilot task~\citep{agirre2012semeval}. As a foundational component of the standard STS evaluation suite, \texttt{STS12} has been consistently used to benchmark sentence representations in both early and recent embedding models~\citep{muennighoff2023mteb,chen2024bge}. Finally, we use the \texttt{IMDb} sentiment classification benchmark—a canonical binary text classification task with 50K labeled movie reviews~\citep{maas2011learning}—frequently employed to assess the transferability of sentence representations in sentiment analysis~\citep{reimers2019sbert,gao2021simcse}. This combination enables rigorous testing across task types, domains, and difficulty levels, ensuring a fair and holistic comparison with prior state-of-the-art approaches that report results on these same standard datasets~\citep{muennighoff2023mteb,enevoldsen2025mmteb,chen2024bge}.




% \begin{table*}[htbp]
% \centering
% \caption{Performance comparison on LoCoMo benchmark (BGE-Small). Each cell shows F1 / BLEU-1 scores.}
% \label{tab:locomo_results_small}
% \renewcommand{\arraystretch}{1.3}
% \resizebox{\textwidth}{!}{%
% \large
% \begin{tabular}{lccccccccccc}
% \toprule
% & \textbf{Method} & \multicolumn{2}{c}{\textbf{Temporal}} & \multicolumn{2}{c}{\textbf{Open-domain}} & \multicolumn{2}{c}{\textbf{Multi-hop}} & \multicolumn{2}{c}{\textbf{Single-hop}} & \multicolumn{2}{c}{\textbf{Average}} \\
% & & F1 & BLEU-1 & F1 & BLEU-1 & F1 & BLEU-1 & F1 & BLEU-1 & F1 & BLEU-1 \\
% \midrule
% MemoryOS & Baseline & 0.4514 & 0.3920 & 0.2834 & 0.2343 & 0.3994 & 0.3048 & 0.5170 & 0.4519 & 0.4672 & 0.3989 \\
%          &  After    & 0.4745 & 0.4072 & 0.3148 & 0.2657 & 0.4208 & 0.3370 & 0.5573 & 0.4920 & 0.4999 & 0.4319 \\
% \cmidrule{1-12}
% Mem0 & Baseline & 0.0738 & 0.0598 & 0.1890 & 0.1388 & 0.2645 & 0.1898 & 0.2743 & 0.2358 & 0.2254 & 0.1846 \\
%      & After    & 0.0974 & 0.0834 & 0.2400 & 0.1826 & 0.2690 & 0.1972 & 0.2937 & 0.2518 & 0.2449 & 0.2024 \\
% \bottomrule
% \end{tabular}%
% }
% \end{table*}



% \begin{table*}[htbp]
% \centering
% \caption{Performance comparison on LoCoMo benchmark (BGE-Small). Each cell shows F1 / BLEU-1 scores.}
% \label{tab:locomo_results_small}
% \renewcommand{\arraystretch}{1.3}
% \resizebox{\textwidth}{!}{%
% \large
% \begin{tabular}{lccccccccccc}
% \toprule
% & \textbf{Setting} & \multicolumn{2}{c}{\textbf{Temporal}} & \multicolumn{2}{c}{\textbf{Open-domain}} & \multicolumn{2}{c}{\textbf{Multi-hop}} & \multicolumn{2}{c}{\textbf{Single-hop}} & \multicolumn{2}{c}{\textbf{Average}} \\
% & & F1 & BLEU-1 & F1 & BLEU-1 & F1 & BLEU-1 & F1 & BLEU-1 & F1 & BLEU-1 \\
% \midrule
% MemoryOS & Baseline & 0.4514 & 0.3920 & 0.2834 & 0.2343 & 0.3994 & 0.3048 & 0.5170 & 0.4519 & 0.4672 & 0.3989 \\
%          & \rowcolor{LightSlateBlue!30} After    & 0.4745 & 0.4072 & 0.3148 & 0.2657 & 0.4208 & 0.3370 & 0.5573 & 0.4920 & 0.4999 & 0.4319 \\  % 第一行After加色
% \cmidrule{1-12}
% Mem0 & Baseline & 0.0738 & 0.0598 & 0.1890 & 0.1388 & 0.2645 & 0.1898 & 0.2743 & 0.2358 & 0.2254 & 0.1846 \\
%      & \rowcolor{LightSlateBlue!30} After    & 0.0974 & 0.0834 & 0.2400 & 0.1826 & 0.2690 & 0.1972 & 0.2937 & 0.2518 & 0.2449 & 0.2024 \\  % 第二行After加色
% \bottomrule
% \end{tabular}%
% }
% \end{table*}


% \begin{table*}[htbp]
%     \centering
%     \caption{Performance comparison on LoCoMo benchmark (BGE-Small). Each cell shows F1 / BLEU-1 scores.}
%     \label{tab:locomo_results_small}
%     \renewcommand{\arraystretch}{1.3}
%     \resizebox{\textwidth}{!}{%
%     \large
%     \begin{tabular}{lccccccccccc}
%     \toprule
%     & \textbf{Setting} & \multicolumn{2}{c}{\textbf{Temporal}} & \multicolumn{2}{c}{\textbf{Open-domain}} & \multicolumn{2}{c}{\textbf{Multi-hop}} & \multicolumn{2}{c}{\textbf{Single-hop}} & \multicolumn{2}{c}{\textbf{Average}} \\
%     & & F1 & BLEU-1 & F1 & BLEU-1 & F1 & BLEU-1 & F1 & BLEU-1 & F1 & BLEU-1 \\
%     \midrule
%     MemoryOS & Baseline & 0.4514 & 0.3920 & 0.2834 & 0.2343 & 0.3994 & 0.3048 & 0.5170 & 0.4519 & 0.4672 & 0.3989 \\
%     \rowcolor{LightSlateBlue!30} & After & 0.4745 & 0.4072 & 0.3148 & 0.2657 & 0.4208 & 0.3370 & 0.5573 & 0.4920 & 0.4999 & 0.4319 \\
%     \cmidrule{1-12}
%     Mem0 & Baseline & 0.0738 & 0.0598 & 0.1890 & 0.1388 & 0.2645 & 0.1898 & 0.2743 & 0.2358 & 0.2254 & 0.1846 \\
%     \rowcolor{LightSlateBlue!30} & After & 0.0974 & 0.0834 & 0.2400 & 0.1826 & 0.2690 & 0.1972 & 0.2937 & 0.2518 & 0.2449 & 0.2024 \\
%     \bottomrule
%     \end{tabular}%
%     }
%     \end{table*}

\begin{table*}[htbp]
    \centering
    \caption{Performance comparison on LoCoMo benchmark (BGE-Small). Each cell shows F1 / BLEU-1 scores.}
    \label{tab:locomo_results_small}
    \renewcommand{\arraystretch}{1.3}
    \resizebox{\textwidth}{!}{%
    \large
    \begin{tabular}{lccccccccccc}
    \toprule
    & \textbf{Setting} & \multicolumn{2}{c}{\textbf{Temporal}} & \multicolumn{2}{c}{\textbf{Open-domain}} & \multicolumn{2}{c}{\textbf{Multi-hop}} & \multicolumn{2}{c}{\textbf{Single-hop}} & \multicolumn{2}{c}{\textbf{Average}} \\
    & & F1 & BLEU-1 & F1 & BLEU-1 & F1 & BLEU-1 & F1 & BLEU-1 & F1 & BLEU-1 \\
    \midrule
    MemoryOS & Baseline & 0.4514 & 0.3920 & 0.2834 & 0.2343 & 0.3994 & 0.3048 & 0.5170 & 0.4519 & 0.4672 & 0.3989 \\
             & \cellcolor{LightSlateBlue!30}After & \cellcolor{LightSlateBlue!30}0.4745 & \cellcolor{LightSlateBlue!30}0.4072 & \cellcolor{LightSlateBlue!30}0.3148 & \cellcolor{LightSlateBlue!30}0.2657 & \cellcolor{LightSlateBlue!30}0.4208 & \cellcolor{LightSlateBlue!30}0.3370 & \cellcolor{LightSlateBlue!30}0.5573 & \cellcolor{LightSlateBlue!30}0.4920 & \cellcolor{LightSlateBlue!30}0.4999 & \cellcolor{LightSlateBlue!30}0.4319 \\
    \cmidrule{1-12}
    Mem0 & Baseline & 0.0738 & 0.0598 & 0.1890 & 0.1388 & 0.2645 & 0.1898 & 0.2743 & 0.2358 & 0.2254 & 0.1846 \\
         & \cellcolor{LightSlateBlue!30}After & \cellcolor{LightSlateBlue!30}0.0974 & \cellcolor{LightSlateBlue!30}0.0834 & \cellcolor{LightSlateBlue!30}0.2400 & \cellcolor{LightSlateBlue!30}0.1826 & \cellcolor{LightSlateBlue!30}0.2690 & \cellcolor{LightSlateBlue!30}0.1972 & \cellcolor{LightSlateBlue!30}0.2937 & \cellcolor{LightSlateBlue!30}0.2518 & \cellcolor{LightSlateBlue!30}0.2449 & \cellcolor{LightSlateBlue!30}0.2024 \\
    \bottomrule
    \end{tabular}%
    }
    \end{table*}



% \begin{table*}[htbp]
% \centering
% \caption{Performance comparison on PERSONAMEM benchmark (BGE-Small).}
% \label{tab:knowme_results}
% \renewcommand{\arraystretch}{1.3}
% \resizebox{\textwidth}{!}{%
% \large
% \begin{tabular}{lccccccccc}
% \toprule
% & \textbf{Setting} & \textbf{Pref. Rec.} & \textbf{Recall Facts} & \textbf{Suggest Ideas} & \textbf{Generalize} & \textbf{Recall Reasons} & \textbf{Track Pref.} & \textbf{Recall Mentioned} & \textbf{Total} \\
% \midrule
% MemoryOS & Baseline & 0.3818 & 0.4754 & 0.0323 & 0.3333 & 0.7980 & 0.5755 & 0.5294 & 0.4092 \\
%          & \rowcolor{LightSlateBlue!30}After    & 0.4545 & 0.4885 & 0.0538 & 0.3158 & 0.7879 & 0.5683 & 0.5294 & 0.4211 \\
% \cmidrule{1-10}
% Mem0 & Baseline & 0.5091 & 0.3377 & 0.1183 & 0.4912 & 0.8384 & 0.5540 & 0.2941 & 0.4669 \\
%      & \rowcolor{LightSlateBlue!30}After    & 0.5091 & 0.3311 & 0.1613 & 0.5088 & 0.8687 & 0.5612 & 0.2941 & 0.4924 \\
% \bottomrule
% \end{tabular}%
% }
% \vspace{1mm}
% \footnotesize
% \end{table*}


\begin{table*}[htbp]
    \centering
    \caption{Performance comparison on PERSONAMEM benchmark (BGE-Small).}
    \label{tab:knowme_results}
    \renewcommand{\arraystretch}{1.3}
    \resizebox{\textwidth}{!}{%
    \large
    \begin{tabular}{lccccccccc}
    \toprule
    & \textbf{Setting} & \textbf{Pref. Rec.} & \textbf{Recall Facts} & \textbf{Suggest Ideas} & \textbf{Generalize} & \textbf{Recall Reasons} & \textbf{Track Pref.} & \textbf{Recall Mentioned} & \textbf{Total} \\
    \midrule
    MemoryOS & Baseline & 0.3818 & 0.4754 & 0.0323 & 0.3333 & 0.7980 & 0.5755 & 0.5294 & 0.4092 \\
             & \cellcolor{LightSlateBlue!30}After & \cellcolor{LightSlateBlue!30}0.4545 & \cellcolor{LightSlateBlue!30}0.4885 & \cellcolor{LightSlateBlue!30}0.0538 & \cellcolor{LightSlateBlue!30}0.3158 & \cellcolor{LightSlateBlue!30}0.7879 & \cellcolor{LightSlateBlue!30}0.5683 & \cellcolor{LightSlateBlue!30}0.5294 & \cellcolor{LightSlateBlue!30}0.4211 \\
    \cmidrule{1-10}
    Mem0 & Baseline & 0.5091 & 0.3377 & 0.1183 & 0.4912 & 0.8384 & 0.5540 & 0.2941 & 0.4669 \\
         & \cellcolor{LightSlateBlue!30}After & \cellcolor{LightSlateBlue!30}0.5091 & \cellcolor{LightSlateBlue!30}0.3311 & \cellcolor{LightSlateBlue!30}0.1613 & \cellcolor{LightSlateBlue!30}0.5088 & \cellcolor{LightSlateBlue!30}0.8687 & \cellcolor{LightSlateBlue!30}0.5612 & \cellcolor{LightSlateBlue!30}0.2941 & \cellcolor{LightSlateBlue!30}0.4924 \\
    \bottomrule
    \end{tabular}%
    }
    \vspace{1mm}
    \footnotesize
    \end{table*}



\subsection{Performance Comparison}
% Performance Comparison Section

% Performance Comparison Section

Table~\ref{tab:locomo_results_small} and Table~\ref{tab:knowme_results} present comprehensive performance comparisons between the baseline \texttt{BGE-small-en-v1.5} model and our fine-tuned variant across LoCoMo and PERSONAMEM benchmarks under both MemoryOS and Mem0 frameworks.

\textbf{LoCoMo Benchmark.} On the LoCoMo benchmark, our fine-tuned model demonstrates consistent improvements across all evaluated scenarios. Under the MemoryOS framework, fine-tuning yields substantial gains: average F1 score increases from 0.4672 to 0.4999 (+3.27\%) and BLEU-1 score improves from 0.3989 to 0.4319 (+3.30\%). The improvements are particularly pronounced in the Single-hop scenario, where F1 and BLEU-1 scores rise from 0.5170/0.4519 to 0.5573/0.4920 (+4.03\%/+4.01\%), and in the Open-domain setting, where F1 improves from 0.2834 to 0.3148 (+3.14\%). Under the Mem0 framework, fine-tuning still delivers meaningful improvements: average F1 increases from 0.2254 to 0.2449 (+1.95\%) and BLEU-1 from 0.1846 to 0.2024 (+1.78\%). Notably, the Open-domain scenario shows the largest absolute improvement, with F1 score increasing from 0.1890 to 0.2400 (+5.10\%).

\textbf{PERSONAMEM Benchmark.} On PERSONAMEM, fine-tuning exhibits differential effects depending on the memory framework. Under MemoryOS, the fine-tuned model achieves a total score of 0.4211, compared to 0.4092 for the baseline (+1.19\%). The most significant improvements are observed in Preference Recommendations (0.3818 $\rightarrow$ 0.4545, +7.27\%) and Suggest New Ideas (0.0323 $\rightarrow$ 0.0538, +2.15\%). Under Mem0, fine-tuning yields more substantial gains: the total score improves from 0.4669 to 0.4924 (+2.55\%). 

\textbf{Cross-Framework Analysis.} The results reveal that fine-tuning benefits both memory frameworks.This suggests that fine-tuning effectively enhances embedding quality regardless of the underlying memory system's sophistication.










% \begin{table*}[htbp]
% \centering
% \caption{Performance comparison on PERSONAMEM benchmark (BGE-Small).}
% \label{tab:knowme_results}
% \renewcommand{\arraystretch}{1.3}
% \resizebox{\textwidth}{!}{%
% \large
% \begin{tabular}{lc|cccccccc}
% \toprule
% & \textbf{Setting} & \textbf{Pref. Rec.} & \textbf{Recall Facts} & \textbf{Suggest Ideas} & \textbf{Generalize} & \textbf{Recall Reasons} & \textbf{Track Pref.} & \textbf{Recall Mentioned} & \textbf{Total} \\
% \midrule
% MemoryOS & Baseline & 0.3818 & 0.4754 & 0.0323 & 0.3333 & 0.7980 & 0.5755 & 0.5294 & 0.4092 \\
%          & After    & 0.4545 & 0.4885 & 0.0538 & 0.3158 & 0.7879 & 0.5683 & 0.5294 & 0.4211 \\
% \cmidrule{1-10}
% Mem0 & Baseline & 0.5091 & 0.3377 & 0.1183 & 0.4912 & 0.8384 & 0.5540 & 0.2941 & 0.4669 \\
%      & After    & 0.5091 & 0.3311 & 0.1613 & 0.5088 & 0.8687 & 0.5612 & 0.2941 & 0.4924 \\
% \bottomrule
% \end{tabular}%
% }
% \vspace{1mm}
% \footnotesize
% \end{table*}

% \subsection{Implementation Details}
% \paragraph{Asynchronous Data Generation Pipeline.}
% We implement an asynchronous processing pipeline to maximize throughput while respecting API rate limits. Key design choices include:
% \begin{itemize}[leftmargin=*,nosep]
%     \item Controlled concurrency with semaphore ($N_{\text{concurrent}}=20$)
%     \item Exponential backoff for rate limit handling
%     \item Incremental saving in JSONL format with file-level locking
% \end{itemize}

% \paragraph{Batch Processing.}
% Conversations are processed in batches of $B=4$ to enable efficient cross-conversation negative sampling while maintaining memory efficiency. This batch size ensures sufficient diversity in easy negatives while keeping API costs manageable.

% \paragraph{Model Training.}
% We fine-tune a pre-trained embedding model using the constructed training data with the following hyperparameters:
% \begin{itemize}[leftmargin=*,nosep]
%     \item Learning rate: $1 \times 10^{-5}$ with linear warmup
%     \item Batch size: 32 with gradient accumulation
%     \item Temperature $\tau$: 0.02
%     \item Training epochs: 3
% \end{itemize}

%上述这个后边放到experiment里





==> latex/record.tex <==
related work
qwen3-embedding https://arxiv.org/abs/2506.05176

M3-Embedding: Multi-Linguality, Multi-Functionality, Multi-Granularity Text Embeddings Through Self-Knowledge Distillation

Modeling Uncertainty in Composed Image Retrieval via Probabilistic Embedding

Hierarchical Level-Wise News Article Clustering via Multilingual Matryoshka Embeddings

Conan-Embedding-v2: Training an LLM from Scratch for Text
Embeddings

In Prospect and Retrospect: Reflective Memory
Management for Long-term Personalized
Dialogue Agents 

PerLTQA: A Personal Long-Term Memory Dataset for Memory
Classification, Retrieval, and Synthesis in Question Answering

Dense Passage Retrieval for Open-Domain Question Answering

UNPACKING THE SUITCASE OF SEMANTIC SIMILARITY

SyNeg: LLM-Driven Synthetic Hard-Negatives for Dense Retrieval

ArcMemo 的关键创新之一是强调“抽象化”，使得“标准的基于嵌入的检索方法（embedding similarity thresholding）”失效

Embedding-based Retrieval Experiments Early in testing, we investigated standard embeddingbased retrieval approaches. Following the ArcMemo-OE setting, we used a VLM-generated caption
to query a vector database of ArcMemo-OE-style concept embeddings. While computationally
cheap compared to autoregressive generation (especially so when leveraging long-form reasoning),
we saw generally poor retrieval results. Using OpenAI’s embeddings API and an o3-mini puzzlesolving backbone proved ineffective, lowering the score from 0.26 to 0.22, marking a 15% reduction.
Qualitative analysis found that retrieved concepts were largely irrelevant to the puzzle and seemed to
over-index on lexical similarity. Moreover, a small set of broadly defined (non-specific) concepts was
found to be grossly overrepresented.


数据构造过程没考虑样本negative难区分度分层(这在记忆检中十分重要)，他们也没考虑自然对话中的不同negtive样本的合理配比，因此导致了难以学到健全的记忆检索功能。-> 消融实验：去掉hard negativem 去掉medium negative. （去掉hard其他补全), discussion base模型结果， discussion MTB benchmark（主表)


(1.洋洋洒洒介绍十几二十个工作)

(2.描述工作异同)

(3.稍微表扬几个比较新比较好的工作)

(4.是否考虑了我们指出的这一点, 指出其存在缺陷)

(话锋一转，我们的工作解决优化了这个缺陷)


实验记录表：
https://odocs.myoas.com/sheets/ZzkLVnzj8yujo53Q/UpmYU
主试验：memoryos-bge-small-knowme
       memoryos-bge-small-locomo
       mem0-bge-small-knowme
       mem0-bge-small-locomo

深绿色为最终结果
浅绿色为没有配比使用全部数据训练的结果

也许可加消融实验：没有hard型数据训练？

其他实验：找几个tasks跑baseline，说明选择这几个tasks的原因




训练样本数: 201462
每 epoch 步数 (batch=512): 393, 选择checkpoint为490步，epoch为1.25个epoch

训练样本数 547577
batchsize = 1024, 选择checkpoint为410步， epoch为0.77 epoch

==> method.tex <==
\section{Method}
%==============================================================================

% We propose \textbf{\method{}}, a \textbf{Hier}archical \textbf{Neg}ative sampling framework for training conversational embedding models. Our approach addresses the overfitting problem in retrieval-oriented dialogue understanding through three key innovations: (1) cross-conversation negative sampling, (2) hierarchical negative stratification, and (3) semantic-aware query generation. \autoref{fig:intro}illustrates our overall pipeline.


We propose HiNS, a Hierarchical Negative sampling framework for training conversational embedding models. Our approach addresses the overfitting problem in retrieval-oriented dialogue understanding through three key innovations: (1) cross-conversation negative sampling, (2) hierarchical negative stratification, and (3) semantic-aware query generation. \autoref{fig:intro} illustrates our overall pipeline. Detailed prompts for each component are provided in Appendix \ref{app:prompts}.

% \begin{figure*}[!ht]
% \vspace{-0.8in}
% \centering
% \includegraphics[height = 0.4\textwidth,width=0.9\textwidth]{latex/pictures/1.pdf}
% \caption{\small
% {\bench} The Hierarchical Negative Sampling process
% }
% \label{fig:intro}
% \vspace{-0.5cm}
% \end{figure*}

\begin{figure*}[!ht]
\vspace{-0.8in}
\centering
\includegraphics[height = 0.42\textwidth,width=0.9\textwidth]{latex/pictures/main1.png}
\caption{\small
 The Hierarchical Negative Sampling process
}
\label{fig:intro}
\vspace{-0.5cm}
\end{figure*}
% \begin{figure*}[!ht]
% \vspace{-0.8in}
% \centering
% \includegraphics[height=0.4\textheight,width=0.9\textwidth]{latex/pictures/1.pdf}
% \caption{\small
% The Hierarchical Negative Sampling process
% }
% \label{fig:intro}
% \vspace{-0.5cm}
% \end{figure*}
% \centering % 临时居中
% \includegraphics[width=0.6\textwidth]{latex/pictures/1.pdf}
% \raggedright % 恢复正文左对齐（避免后续文本也居中）
% \includegraphics[width=1\textwidth]{latex/pictures/1.pdf} illustrates our overall pipeline.


%------------------------------------------------------------------------------
\subsection{Problem Formulation}
%------------------------------------------------------------------------------

Given a multi-turn conversation $\mathcal{C} = \{m_1, m_2, \ldots, m_T\}$ between two participants $P_1$ and $P_2$, and a natural language query $q$, our goal is to learn an embedding function $f_\theta$ such that:
\begin{equation}
\text{sim}(f_\theta(q), f_\theta(m^+)) > \text{sim}(f_\theta(q), f_\theta(m^-))
\end{equation}
where $m^+$ denotes relevant messages and $m^-$ denotes irrelevant messages. The key challenge lies in constructing informative negative samples that prevent the model from learning superficial shortcuts.

%------------------------------------------------------------------------------
\subsection{Persona-Grounded Conversation Synthesis}
%------------------------------------------------------------------------------

To generate diverse and realistic training conversations, we design a persona-grounded synthesis pipeline.

\paragraph{Persona Sampling.}
For each conversation, we sample two distinct participants from a large-scale persona database (Nvidia Nemotron Personas). Each persona $\mathcal{P}_i$ comprises two attribute sets: (1) basic attributes $\mathcal{B}_i$ including demographics (sex, age, marital status), education (level, field), and location (city, state, country), and (2) personality attributes $\mathcal{A}_i$ including professional persona, interests (sports, arts, travel, culinary), skills, hobbies, and career goals. To ensure diversity while maintaining computational efficiency, we randomly sample $k=3$ personality attributes per persona:
% \begin{equation}
% \mathcal{P}_i = \{\mathcal{B}_i, \mathcal{A}_i\}, \quad \mathcal{A}_i \sim \text{RandomSample}(\mathcal{A}_{\text{all}}, k=3)
% \end{equation}
\begin{equation}
\begin{aligned}
\mathcal{P}_i &= \{\mathcal{B}_i, \mathcal{A}_i\}, \\
\mathcal{A}_i &\sim \text{RandomSample}(\mathcal{A}_{\text{all}}, k=3)
\end{aligned}
\end{equation}
where $\mathcal{A}_{\text{all}}$ denotes all available personality attributes. This sampling strategy ensures each conversation involves distinct personas with varied characteristics.

\paragraph{Event Generation.}
Rather than directly exposing personality traits, we generate naturalistic daily events $\mathcal{E}_i$ that implicitly reflect the persona. For each participant $P_i$ with name $\text{name}_i$, we generate exactly 6 events using an LLM:
\begin{equation}
\mathcal{E}_i = \{\text{event}_1, \ldots, \text{event}_6\} = \text{LLM}(\mathcal{B}_i, \mathcal{A}_i, \text{name}_i)
\end{equation}
Each event $\text{event}_j$ is a natural language description of 10--25 words, covering four categories: (1) routine activities, (2) social interactions, (3) hobbies and interests, and (4) mundane daily tasks. Critically, events use the person's actual name (not generic pronouns like ``He/She'') and are not required to explicitly reference all persona attributes. We deliberately limit to 6 events to reduce information density and avoid overly structured patterns that could lead to shortcut learning.

\paragraph{Natural Conversation Generation.}
The conversation is synthesized as a 20-turn dialogue (40 messages total) between $P_1$ and $P_2$. Each message $m_t$ is structured as a tuple $(\text{speaker}, \text{message})$, where $\text{speaker} \in \{P_1, P_2\}$ and $\text{message}$ is the text content. The conversation generation follows:
\begin{equation}
\mathcal{C} = \{m_1, \ldots, m_{40}\} = \text{LLM}(\mathcal{E}_1, \mathcal{E}_2, \text{brief}_1, \text{brief}_2)
\end{equation}
where $\text{brief}_i$ is a semantic description ( ``eg. the retired aerospace engineer who loves gardening'') generated from $\mathcal{B}_i$ and $\mathcal{A}_i$. The generation process enforces natural flow by: (1) not requiring every message to reference a specific event, (2) including greetings, reactions, and transitions, and (3) varying message lengths (5--40 words). This design prevents the model from learning identity-based shortcuts while maintaining realistic dialogue structure.

%------------------------------------------------------------------------------
\subsection{Hierarchical Negative Sampling}
%------------------------------------------------------------------------------

We introduce a three-tier negative sampling strategy based on semantic distance to the positive samples. This hierarchy enables the model to learn fine-grained distinctions rather than relying on superficial features.

% \begin{definition}
% Given a query $q$ targeting person $P_t$ on topic $\tau$, we define three negative categories:
% \begin{itemize}[leftmargin=*,nosep]
%     \item \textbf{Hard Negatives} $\mathcal{N}_h$: Messages from the same conversation, same topic $\tau$, but different speaker $P_{\bar{t}}$
%     \item \textbf{Medium Negatives} $\mathcal{N}_m$: Messages from the same conversation but different topics $\tau' \neq \tau$
%     \item \textbf{Easy Negatives} $\mathcal{N}_e$: Messages from entirely different conversations
% \end{itemize}
% \end{definition}


\noindent Given a query $q$ targeting person $P_t$ on topic $\tau$, we define three negative categories:
\begin{itemize}[leftmargin=*,nosep]
    \item \textbf{Hard Negatives} $\mathcal{N}_h$: Messages from the same conversation, same topic $\tau$, but different speaker $P_{\bar{t}}$
    \item \textbf{Medium Negatives} $\mathcal{N}_m$: Messages from the same conversation but different topics $\tau' \neq \tau$
    \item \textbf{Easy Negatives} $\mathcal{N}_e$: Messages from entirely different conversations
\end{itemize}


Formally, for a query $q$ with evidence set $\mathcal{V} \subset \mathcal{C}$ (positive message IDs) and target person $P_t$ on topic $\tau$, we construct negatives as follows. Let $\mathcal{M} = \mathcal{C} \setminus \mathcal{V}$ denote all non-evidence messages in the conversation.

\textbf{Hard Negatives:} We first identify candidate messages from $\mathcal{M}$ that share the same topic $\tau$ but are spoken by a different person:
% \begin{equation}
% \mathcal{N}_h^{\text{candidate}} = \{m \in \mathcal{M} : \text{topic}(m) = \tau, \text{speaker}(m) \neq P_t\}
% \end{equation}

\begin{equation}
\scalebox{0.9}{$\mathcal{N}_h^{\text{candidate}} = \{m \in \mathcal{M} : \text{topic}(m) = \tau, \text{speaker}(m) \neq P_t\}$}
\end{equation}

We then randomly sample from $\mathcal{N}_h^{\text{candidate}}$ with a cap of $2 \times |\mathcal{V}|$:
\begin{equation}
\scalebox{0.9}{$\mathcal{N}_h = \text{RandomSample}(\mathcal{N}_h^{\text{candidate}}, \min(|\mathcal{N}_h^{\text{candidate}}|, 2|\mathcal{V}|))$}
\end{equation}
% \begin{equation}
% \mathcal{N}_h = \text{RandomSample}(\mathcal{N}_h^{\text{candidate}}, \min(|\mathcal{N}_h^{\text{candidate}}|, 2|\mathcal{V}|))
% \end{equation}

\textbf{Medium Negatives:} From the remaining non-evidence messages that are not hard negatives:
\begin{equation}
\mathcal{N}_m^{\text{candidate}} = \mathcal{M} \setminus \mathcal{N}_h
\end{equation}
We sample up to $|\mathcal{V}|$ messages:
\begin{equation}
\scalebox{0.9}{$\mathcal{N}_m = \text{RandomSample}(\mathcal{N}_m^{\text{candidate}}, \min(|\mathcal{N}_m^{\text{candidate}}|, |\mathcal{V}|))$}
\end{equation}

% \begin{equation}
% \mathcal{N}_m = \text{RandomSample}(\mathcal{N}_m^{\text{candidate}}, \min(|\mathcal{N}_m^{\text{candidate}}|, |\mathcal{V}|))
% \end{equation}

\textbf{Easy Negatives:} For conversation $\mathcal{C}_i$ in batch $\mathcal{G}$, we collect messages from all other conversations:
\begin{equation}
\mathcal{N}_e^{(i)} = \bigcup_{j \neq i} \{m : m \in \mathcal{C}_j\}
\end{equation}
and sample up to $|\mathcal{V}|$ messages:
\begin{equation}
\mathcal{N}_e = \text{RandomSample}(\mathcal{N}_e^{(i)}, \min(|\mathcal{N}_e^{(i)}|, |\mathcal{V}|))
\end{equation}

\paragraph{Batch-wise Cross-Conversation Sampling.}
To efficiently construct $\mathcal{N}_e$, we process conversations in batches of size $B=4$. This batch-level processing enables efficient sharing of messages across conversations for easy negative sampling while maintaining computational efficiency.

% \paragraph{Negative Ratio Control.}
% The sampling strategy described above naturally yields a ratio of approximately $|\mathcal{N}_h| : |\mathcal{N}_m| : |\mathcal{N}_e| \approx 2 : 1 : 1$ when sufficient candidates are available. The total number of negatives per query is capped at $4 \times |\mathcal{V}|$, maintaining a positive-negative ratio of approximately 1:4, which balances learning signal strength with computational efficiency.

%------------------------------------------------------------------------------
\subsection{Semantic Query Generation}
%------------------------------------------------------------------------------

We propose semantic query generation with three key designs.


\paragraph{Descriptive Person Reference.}
For each participant $P_i$, we generate a semantic \textit{person brief} $\text{brief}_i$ (15--25 words) that combines demographic/occupational traits with interests:
\begin{equation}
\text{brief}_i = \text{LLM}(\text{name}_i, \mathcal{B}_i, \mathcal{A}_i)
\end{equation}
Examples include ``the retired aerospace engineer who loves gardening and historical fiction'' or ``the young Atlanta-based yoga enthusiast and aspiring chef''. During query generation, the LLM receives the conversation $\mathcal{C}$ along with participant information $(P_1, \text{brief}_1)$ and $(P_2, \text{brief}_2)$, and generates queries that reference participants using their names (e.g., ``What hobbies does James mention?'') or brief-derived descriptive phrases (e.g., ``How does the retired teacher spend weekends?'').





% \paragraph{Descriptive Person Reference.}
% Queries use semantic descriptions generated by an LLM:
% \begin{equation}
% \text{ref}(P_i) = \text{LLM}(\mathcal{B}_i, \mathcal{A}_i)
% \end{equation}
% For example, this produces references like ``the young Atlanta-based yoga enthusiast''.


% For each participant $P_i$, we generate a \textit{person brief} $\text{brief}_i$ that serves as a semantic identifier. The brief generation follows a structured prompt-based approach:
% \begin{equation}
% \text{brief}_i = \text{LLM}(\text{Prompt}_{\text{brief}}(\mathcal{B}_i, \mathcal{A}_i, \text{name}_i))
% \end{equation}
% where $\text{Prompt}_{\text{brief}}$ constructs a prompt template that specifies: (1) input format: the person's name, basic attributes $\mathcal{B}_i$ (demographics, education, location), and personality attributes $\mathcal{A}_i$ (interests, skills, goals), (2) output requirements: a concise 15--25 word description that is unique, identifiable, and natural to use in questions, (3) content constraints: the description must mention 2--3 key traits, typically combining one demographic/occupational trait (age, occupation, location) with 1--2 interests or hobbies, and (4) format constraints: output only the description text without quotes or additional formatting.

% The generated briefs take forms such as ``the retired aerospace engineer who loves gardening and historical fiction'' or ``the young Atlanta-based yoga enthusiast and aspiring chef''. These briefs are then used as input to the query generation process alongside the conversation and participant names.

% During query generation, the LLM receives the conversation $\mathcal{C}$ along with participant information formatted as:
% \begin{equation}
% \text{QueryInput} = \{\mathcal{C}, (P_1, \text{brief}_1), (P_2, \text{brief}_2)\}
% \end{equation}
% The query generation prompt $\text{Prompt}_{\text{query}}$ explicitly instructs the LLM to use semantic identification: queries should reference participants using either (1) their actual names (e.g., ``What hobbies does James mention?''), (2) descriptive phrases derived from the briefs (e.g., ``How does the retired teacher spend weekends?''), or (3) combinations of name and brief attributes. The prompt explicitly prohibits generic labels like ``user1'' or ``user2''. This results in queries that naturally incorporate semantic person references, such as:
% \begin{equation}
% q = \text{LLM}(\text{Prompt}_{\text{query}}(\text{QueryInput}))
% \end{equation}
% where each generated query $q$ contains a $\text{query\_text}$ field that uses semantic person references rather than generic identifiers.




\paragraph{Topic-Aware Query Generation.}
We generate queries through a two-stage process. First, we perform topic clustering on the conversation to identify $K$ main topics:
\begin{equation}
\mathcal{T} = \text{TopicCluster}(\mathcal{C}) = \{(\tau_k, \mathcal{M}_1^k, \mathcal{M}_2^k)\}_{k=1}^{K}
\end{equation}
where $\mathcal{M}_j^k$ denotes the set of message IDs from participant $P_j$ on topic $\tau_k$. Then, we generate exactly 6 queries $\mathcal{Q} = \{q_1, \ldots, q_6\}$ using an LLM, ensuring balanced coverage:
\begin{itemize}[leftmargin=*,nosep]
    \item 2 queries targeting $P_1$'s activities and interests
    \item 2 queries targeting $P_2$'s activities and interests  
    \item 2 queries about shared topics or interactions between both participants
\end{itemize}
Each query $q_i$ is associated with: (1) $\text{query\_text}$: the natural language query, (2) $\text{target\_person}$: $P_1$ or $P_2$, (3) $\text{topic}$: the primary topic $\tau_k$, and (4) $\text{evidence}$: a set of message IDs $\mathcal{V}_i \subset \mathcal{C}$ that directly answer the query.

\paragraph{Evidence Calibration.}
For each query, the evidence set $\mathcal{V}_i$ contains 5--12 message IDs, carefully calibrated to avoid both sparse supervision (too few positives leading to weak learning signals) and noisy labels (too many loosely related messages that dilute the positive signal). The evidence messages are primarily from the target person's messages on the relevant topic.

%------------------------------------------------------------------------------
\subsection{Training Objective}
%------------------------------------------------------------------------------

For each query $q$ with evidence set $\mathcal{V}$, we construct training triplets:
% \begin{equation}
% \mathcal{D} = \{(q, m^+, \{n_1, \ldots, n_K\}) : m^+ \in \mathcal{V}, n_k \in \mathcal{N}_h \cup \mathcal{N}_m \cup \mathcal{N}_e\}
% \end{equation}

\begin{equation}
\begin{split}
\mathcal{D} = \{(q, m^+, \{n_1, \ldots, n_K\}) : {} \\
m^+ \in \mathcal{V}, n_k \in \mathcal{N}_h \cup \mathcal{N}_m \cup \mathcal{N}_e\}
\end{split}
\end{equation}

The final training objective follows the InfoNCE loss~\cite{oord2018representation} with hierarchical negatives.
% \begin{equation}
% \mathcal{L} = -\log \frac{\exp(\text{sim}(q, m^+)/\tau)}{\exp(\text{sim}(q, m^+)/\tau) + \sum_{k=1}^{K} \exp(\text{sim}(q, n_k)/\tau)}
% \label{eq:loss}
% \end{equation}

% \begin{equation}
% \scalebox{1}{$\mathcal{L} = -\log \frac{\exp(\text{sim}(q, m^+)/\tau)}{\exp(\text{sim}(q, m^+)/\tau) + \sum_{k=1}^{K} \exp(\text{sim}(q, n_k)/\tau)}$}
% \label{eq:loss}
% \end{equation}
% \begin{minipage}{0.2\textwidth}
% \begin{equation}
% \mathcal{L} = -\log \frac{\exp(\text{sim}(q, m^+)/\tau)}{\exp(\text{sim}(q, m^+)/\tau) + \sum_{k=1}^{K} \exp(\text{sim}(q, n_k)/\tau)}
% \label{eq:loss}
% \end{equation}
% \end{minipage}
% where $\tau$ is the temperature hyperparameter and $\text{sim}$ denotes cosine similarity between embeddings.

% \subsection{Implementation Details}
% \paragraph{Algorithm Overview.}
% Algorithm~\ref{alg:hierneg} summarizes the complete hierarchical negative sampling procedure. Given a batch of $B$ conversations $\mathcal{G} = \{\mathcal{C}_1, \ldots, \mathcal{C}_B\}$, the algorithm processes each conversation as follows: (1) Topic clustering identifies main topics $\mathcal{T}_i$ (Line 3), (2) Semantic queries $\mathcal{Q}_i$ are generated with evidence sets (Line 4), (3) Cross-conversation messages are collected for easy negatives $\mathcal{N}_e^{(i)}$ (Line 5). For each query $q \in \mathcal{Q}_i$, the algorithm extracts the evidence set $\mathcal{V}$, target person $P_t$, and topic $\tau$ (Line 7), then constructs three negative types: hard negatives $\mathcal{N}_h$ from same-topic but different-speaker messages (Line 8), medium negatives $\mathcal{N}_m$ from different topics (Line 9), and easy negatives sampled from $\mathcal{N}_e^{(i)}$ (Line 10). The sampling follows ratio $2:1:1$ with caps as described above (Line 10). Finally, training triplets are assembled by pairing each positive message $m^+ \in \mathcal{V}$ with the combined negative set (Lines 11--13).


% \begin{algorithm}[!htbp]
% \caption{Hierarchical Negative Sampling}
% \label{alg:hierneg}
% \begin{algorithmic}[1]
% \REQUIRE Conversation batch $\mathcal{G} = \{\mathcal{C}_1, \ldots, \mathcal{C}_B\}$
% \ENSURE Training samples $\mathcal{D}$
% \STATE $\mathcal{D} \leftarrow \emptyset$
% \FOR{each conversation $\mathcal{C}_i \in \mathcal{G}$}
%     \STATE $\mathcal{T}_i \leftarrow \text{TopicCluster}(\mathcal{C}_i)$
%     \STATE $\mathcal{Q}_i \leftarrow \text{GenerateQueries}(\mathcal{C}_i, \mathcal{T}_i)$
%     \STATE $\mathcal{N}_e^{(i)} \leftarrow \bigcup_{j \neq i} \text{Messages}(\mathcal{C}_j)$
%     \FOR{each query $q \in \mathcal{Q}_i$}
%         \STATE Extract evidence set $\mathcal{V}$, target person $P_t$, topic $\tau$
%         \STATE $\mathcal{M} \leftarrow \mathcal{C}_i \setminus \mathcal{V}$ \COMMENT{Non-evidence messages}
%         \STATE $\mathcal{N}_h^{\text{cand}} \leftarrow \{m \in \mathcal{M} : \text{topic}(m) = \tau, \text{speaker}(m) \neq P_t\}$
%         \STATE $\mathcal{N}_h \leftarrow \text{RandomSample}(\mathcal{N}_h^{\text{cand}}, \min(|\mathcal{N}_h^{\text{cand}}|, 2|\mathcal{V}|))$
%         \STATE $\mathcal{N}_m^{\text{cand}} \leftarrow \mathcal{M} \setminus \mathcal{N}_h$
%         \STATE $\mathcal{N}_m \leftarrow \text{RandomSample}(\mathcal{N}_m^{\text{cand}}, \min(|\mathcal{N}_m^{\text{cand}}|, |\mathcal{V}|))$
%         \STATE $\mathcal{N}_e \leftarrow \text{RandomSample}(\mathcal{N}_e^{(i)}, \min(|\mathcal{N}_e^{(i)}|, |\mathcal{V}|))$
%         \FOR{each positive $m^+ \in \mathcal{V}$}
%             \STATE $\mathcal{D} \leftarrow \mathcal{D} \cup \{(q, m^+, \mathcal{N}_h \cup \mathcal{N}_m \cup \mathcal{N}_e)\}$
%         \ENDFOR
%     \ENDFOR
% \ENDFOR
% \RETURN $\mathcal{D}$
% \end{algorithmic}
% \end{algorithm}

==> relatedwork.tex <==
\section{Related Work}

\subsection{Memory-Augmented Dialogue Agents}

% Agent system has been a popular research in the recent year \cite{li2025chain}. Multiple memory systems and benchmarks have been raised in recent years \cite{wang2025mem,liang2025towards}.   Recent years have witnessed significant advances in memory-augmented dialogue agents. To support personalization and consistency in long-term interactions, substantial research efforts have focused on mechanisms for memory storage, indexing, and retrieval. Representative studies include \textbf{PerLTQA}\citep{du2024perltqa}, which introduced the first QA benchmark dataset tailored for personalized long-term memory; \textbf{In Prospect and Retrospect} \citep{tan2025prospect}, which proposed a reflective memory management framework that dynamically filters outdated or conflicting memories; and \textbf{ArcMemo} \citep{ho2025arcmemo}, which emphasizes \emph{abstracted} memory representations and demonstrates that standard embedding-similarity--based retrieval becomes ineffective at higher levels of abstraction. Additional contributions include \textbf{ChatDB} \cite{hu2023chatdb}, which improves long-term consistency by decoupling user facts from dialogue history through a structured memory store.

% Recent years have witnessed significant advances in memory-augmented dialogue agents \citep{wang2025xxx, liang2025xxx, li2025xxx, zhang2025a}. \citet{hu2025memory} provide a comprehensive survey of memory mechanisms in modern AI agents, systematically analyzing challenges in storage, retrieval, and reasoning. To support personalization and consistency in long-term interactions, substantial research efforts have focused on mechanisms for memory storage, indexing, and retrieval. Representative studies include PerLTQA \citep{du2024xxx}, which introduced the first QA benchmark dataset tailored for personalized long-term memory; In Prospect and Retrospect \citep{tan2025xxx}, which proposed a reflective memory management framework that dynamically filters outdated or conflicting memories; and ArcMemo \citep{ho2025xxx}, which emphasizes abstracted memory representations and demonstrates that standard embedding-similarity-based retrieval becomes ineffective at higher levels of abstraction. Additional contributions include ChatDB \citep{hu2023xxx}, which improves long-term consistency by decoupling user facts from dialogue history through a structured memory store; Reflexion \citep{shinn2023xxx}, which incorporates a language-based reflection mechanism that enables agents to autonomously correct erroneous memories.




Recent years have witnessed significant advances in memory-augmented dialogue agents \cite{wang2025mem,liang2025towards,li2025chain,zhang2025memevolve}. \cite{hu2025memory} provide a comprehensive survey of agent memory systems, analyzing memory from the perspectives of forms (token-level, parametric, latent), functions (factual, experiential, working), and dynamics (formation, evolution, retrieval).To support personalization and consistency in long-term interactions, substantial research efforts have focused on mechanisms for memory storage, indexing, and retrieval. Representative studies include \textbf{PerLTQA}\citep{du2024perltqa}, which introduced the first QA benchmark dataset tailored for personalized long-term memory; \textbf{In Prospect and Retrospect} \citep{tan2025prospect}, which proposed a reflective memory management framework that dynamically filters outdated or conflicting memories; and \textbf{ArcMemo} \citep{ho2025arcmemo}, which emphasizes \emph{abstracted} memory representations and demonstrates that standard embedding-similarity--based retrieval becomes ineffective at higher levels of abstraction. Additional contributions include \textbf{ChatDB} \cite{hu2023chatdb}, which improves long-term consistency by decoupling user facts from dialogue history through a structured memory store; \textbf{Reflexion} \cite{shinn2023reflexion}, which incorporates a language-based reflection mechanism that enables agents to autonomously correct erroneous memories. However, existing memory-augmented systems commonly overlook the empirically observed \emph{difficulty spectrum} and distributional patterns of negative samples when training their retrieval embedding models. As highlighted by studies such as \textbf{LongMem} \cite{wang2023augmenting}, errors in real dialogues exhibit a structured difficulty distribution across easy, medium, and hard categories. This oversight results in models with insufficient discriminative power against ``hard'' distractors that are semantically similar but factually contradictory, thereby undermining their capacity to sustain consistent, personalized dialogue over extended interactions.

% However, existing memory-augmented systems commonly overlook the empirically observed \emph{difficulty spectrum} and distributional patterns of negative samples when training their retrieval embedding models. As highlighted by studies such as \textbf{LongMem} \cite{wang2023augmenting}, memory errors in real dialogues exhibit a structured difficulty distribution with relatively stable frequencies across easy, medium, and hard categories. This oversight results in models with insufficient discriminative power against ``hard'' distractors that are semantically similar but factually contradictory, thereby undermining their capacity to sustain consistent, personalized dialogue over extended interactions.

\subsection{Text Embedding Models}

Models such as \textbf{GTE} \cite{li2023towards} enhance generalization through instruction tuning; \textbf{BGE} \cite{xiao2024c} leverages contrastive learning and large-scale alignment to refine embedding quality; \textbf{M3-Embedding} \cite{chen2024bge} employs self-knowledge distillation to support multi-granularity, multilingual, and multifunctional embeddings; and \textbf{Qwen3 Embedding} \cite{zhang2025qwen3} builds upon the Qwen3 foundation model with a multi-stage training pipeline: it first uses LLMs to synthesize high-quality, cross-lingual, and cross-domain training pairs, then applies model merging strategies to boost robustness.

\subsubsection{Hard Negative Sampling}

Hard negative sampling, a key technique for text embedding and dense retrieval, encompasses static (predefined via data/model, e.g., \cite{he2023learning,lin2020world,ren2021rocketqav2}) and dynamic (adaptive to model state, e.g., \cite{guu2020retrieval,zhan2021optimizing}; \textbf{EDHNS} \cite{han2024efficient}) paradigms that recognize negative sample heterogeneity and use model-derived similarities for difficulty categorization to boost model discrimination.


\subsubsection{Dense Retrieval Methods}

\textbf{DPR} \cite{karpukhin2020dense} established an end-to-end dense retrieval paradigm for open-domain QA using a dual-encoder architecture; \textbf{ANCE} \cite{xiong2020approximate} enables dynamic hard negative sampling via asynchronous index updates; \textbf{RocketQA} \cite{qu2021rocketqa} improves training stability with a denoised negative selection mechanism; \textbf{SyNeg} \cite{li2024syneg} leverages LLMs to generate semantically challenging hard negatives, thereby enhancing sensitivity to subtle semantic distinctions.

However, these approaches have fundamental limitations in negative sampling design. \textbf{General-purpose embedding models} (e.g., GTE, BGE, Qwen3 Embedding) treat negatives as homogeneous noise, using heuristically fixed ratios without explicit difficulty stratification. \textbf{Dense retrieval methods} (e.g., DPR, ANCE, SyNeg) adopt the "harder is better" paradigm, ignoring the continuous difficulty spectrum and co-occurrence patterns of negatives in real interactions. \textbf{Hard negative sampling} approaches, meanwhile, define difficulty via model-derived similarities, lacking empirical grounding in real dialogue error distributions.
Collectively, these limitations hinder embedding models from disambiguating semantically proximal but factually conflicting memory distractors in long-horizon interactions, resulting in weak discriminative power, poor retrieval robustness, and compromised dialogue consistency under structured memory errors.
To address these, we propose a stratified negative sampling framework. By modeling real dialogue difficulty distribution explicitly, it enhances retrieval accuracy under complex interference and improves downstream performance.


==> testtable.tex <==
\newpage
% 彻底清除页面顶部所有默认间距（核心修改）
\vspace*{-1cm}  % 强制上移，可根据实际排版微调数值（如-1.8cm/-2.2cm）
\noindent  % 取消段落首行缩进
\begin{table*}[!t]  % !H 强制固定位置，完全禁用浮动（最顶优先级）
    \centering
    \caption{General embedding benchmark comparison: Baseline(BGE-Small) vs After fine tuning .}
    \label{tab:mteb_comparison}
    \renewcommand{\arraystretch}{1.2}
    \resizebox{\textwidth}{!}{%
    \small
    \begin{tabular}{lccccl}
    \toprule
    \textbf{Task Name} & \textbf{Baseline} & \textbf{After} & \textbf{Diff.} & \textbf{Diff. (\%)} & \textbf{Status} \\
    \midrule
    TwentyNewsgroupsClustering & 0.349190 & 0.369433 & +0.020243 & +5.80\% & \checkmark \\
    ArXivHierarchicalClusteringS2S & 0.532609 & 0.552233 & +0.019624 & +3.68\% & \checkmark \\
    StackExchangeClusteringP2P.v2 & 0.383960 & 0.385161 & +0.001201 & +0.31\% & \checkmark \\
    STS12 & 0.658655 & 0.655377 & -0.003278 & -0.50\% & $\times$ \\
    ImdbClassification & 0.878528 & 0.862592 & -0.015936 & -1.81\% & $\times$ \\
    \bottomrule
    \end{tabular}%
    }
\end{table*}

% \newpage
% \begin{table*}[htbp]
%     \centering
%     \caption{General embedding benchmark comparison: Baseline(BGE-Small) vs After fine tuning .}
%     \label{tab:mteb_comparison}
%     \renewcommand{\arraystretch}{1.2}
%     \resizebox{\textwidth}{!}{%
%     \small
%     \begin{tabular}{lccccl}
%     \toprule
%     \textbf{Task Name} & \textbf{Baseline} & \textbf{After} & \textbf{Diff.} & \textbf{Diff. (\%)} & \textbf{Status} \\
%     \midrule
%     TwentyNewsgroupsClustering & 0.349190 & 0.369433 & +0.020243 & +5.80\% & \checkmark \\
%     ArXivHierarchicalClusteringS2S & 0.532609 & 0.552233 & +0.019624 & +3.68\% & \checkmark \\
%     StackExchangeClusteringP2P.v2 & 0.383960 & 0.385161 & +0.001201 & +0.31\% & \checkmark \\
%     STS12 & 0.658655 & 0.655377 & -0.003278 & -0.50\% & $\times$ \\
%     ImdbClassification & 0.878528 & 0.862592 & -0.015936 & -1.81\% & $\times$ \\
%     \bottomrule
%     \end{tabular}%
%     }
%     \end{table*}


% \clearpage
% \begin{center}
% \captionsetup{justification=centering}
% \captionof{table}{General embedding benchmark comparison: Baseline(BGE-Small) vs After fine tuning.}
% \label{tab:mteb_comparison}
% \renewcommand{\arraystretch}{1.2}
% \resizebox{\textwidth}{!}{%
% \small
% \begin{tabular}{lccccl}
% \toprule
% \textbf{Task Name} & \textbf{Baseline} & \textbf{After} & \textbf{Diff.} & \textbf{Diff. (\%)} & \textbf{Status} \\
% \midrule
% TwentyNewsgroupsClustering & 0.349190 & 0.369433 & +0.020243 & +5.80\% & \checkmark \\
% ArXivHierarchicalClusteringS2S & 0.532609 & 0.552233 & +0.019624 & +3.68\% & \checkmark \\
% StackExchangeClusteringP2P.v2 & 0.383960 & 0.385161 & +0.001201 & +0.31\% & \checkmark \\
% STS12 & 0.658655 & 0.655377 & -0.003278 & -0.50\% & $\times$ \\
% ImdbClassification & 0.878528 & 0.862592 & -0.015936 & -1.81\% & $\times$ \\
% \bottomrule
% \end{tabular}%
% }
% \end{center}




